Big-Bang Nucleosynthesis

A critical review is given of the current status of cosmological nucleosynthesis. In the framework of the Standard Model with 3 types of relativistic neutrinos, the baryon-to-photon ratio, $\eta$, corresponding to the inferred primordial abundances of deuterium and helium-4 is consistent with the independent determination of $\eta$ from observations of anisotropies in the cosmic microwave background. However the primordial abundance of lithium-7 inferred from observations is significantly below its expected value. Taking systematic uncertainties in the abundance estimates into account, there is overall concordance in the range $\eta = (5.7-6.7)\times 10^{-10}$ at 95% CL (corresponding to a cosmological baryon density $\Omega_B h^2 = 0.021 - 0.025$). The D and He-4 abundances, when combined with the CMB determination of $\eta$, provide the bound $N_\nu=3.28 \pm 0.28$ on the effective number of neutrino species. Other constraints on new physics are discussed briefly.

==> bigbangnuc-allref.tex <==
\referencelist

\reference{wfh} R.V.~Wagoner \etal,
\aj148,3(1967) 
\endreference
%%CITATION = ASJOA,148,3;%%
%\reference{*wag} R.V.~Wagoner
%\aj179,343(1973)
%\endreference

%\reference{wssok} T.P.~Walker \etal,
%\aj376,51(1991)
%\endreference

%\reference{mm} R.A.~Malaney and G.J.~Mathews,
%\prept229,145(1993) 
%\endreference
%%CITATION = PRPLC,229,145;%%

\reference{st} D.N.~Schramm and M.S.~Turner,
\rmp70,303(1998)
\endreference
%%CITATION = ASTRO-PH/9706069;%%

% \reference{osw} K.A.~Olive \etal, 
% \prept333,389(2000) 
% \endreference
%%CITATION = ASTRO-PH/9905320;%%

\reference{steigman} G.~Steigman,
\arnps57,463(2007)
\endreference

\reference{iocco} F.~Iocco \etal,
\prept472,1(2009)
\endreference

\reference{sar} S.~Sarkar,
\rpp59,1493(1996)
\endreference
%%CITATION = HEP-PH/9602260;%%

\reference{jedpos} K.~Jedamzik and M.~Pospelov,
{\rm New J.\ Phys. } {\bf 11}, 105028 (2009)
\endreference

\reference{pospra} M.~Pospelov and J.~Pradler,
\arnps60,539(2010)
\endreference

\reference{fie11} B.D.~Fields, 
\arnps61,47(2011)
\endreference

\reference{peeb} P.J.E.~Peebles,
\prl16,411(1966)
\endreference
%\reference{*shv} V.F.~Shvartsman,
%\jetpl9,184(1969)
%\endreference

\reference{bbf} J.~Bernstein \etal, 
\rmp61,25(1989)
\endreference
%%CITATION = RMPHA,61,25;%%

\reference{m} S.~Mukhanov,
{Int.~J.~Theor.~Phys.}~{\bf 143}, 669 (2004)
\endreference

\reference{esd} R.~Esmailzadeh \etal,
\aj378,504(1991)
\endreference

\reference{cfo5} R.H.~Cyburt \etal,
{JCAP}~{\bf 0811}, 012 (2008)
\endreference

\reference{cfo} R.H.~Cyburt \etal,
{New Astron.}~{\bf 6}, 215 (2001)
\endreference

\reference{kaw} L.~Kawano,
FERMILAB-PUB-92/04-A
\endreference

%\reference{sark}
%{\tt http://www-thphys.physics.ox.ac.uk/users/\break
%SubirSarkar/bbn.html\rm}
%\endreference

\reference{parthenope} O.~Pisanti \etal,
{Comput.~Phys.~Commun.}~{\bf 178}, 956 (2008)
\endreference

\reference{alterBBN} A.~Arbey,
{\tt arXiv:1106.1363}\rm
\endreference

%\reference{dic} D.A.~Dicus \etal,
%\prD26,2694(1982)
%\endreference
\reference{emmp} S.~Esposito \etal,
\npB568,421(2000)
\endreference

\reference{dt} S.~Dodelson and M.S.~Turner,
\prD46,3372(1992)
\endreference

\reference{seckel} D.~Seckel,
{\tt hep-ph/9305311}\rm
\endreference
\reference{*lt} R.~Lopez and M.S.~Turner, 
\prD59,103502(1999)
\endreference

%\reference{kr} L.M.~Krauss and P.~Romanelli,
%\aj358,47(1990)
%\endreference

\reference{skm} M.S.~Smith \etal,
\ajs85,219(1993)
\endreference

%\reference{kk} L.M.~Krauss and P.~Kernan,
%\ajl432,L79(1994)
%\endreference


\reference{flsv} G.~Fiorentini \etal,
\prD58,063506(1998)
\endreference

\reference{coc} A.~Coc \etal,
\aj744,158(2012)
\endreference

\reference{nb} K.M.~Nollett and S.~Burles,
\prD61,123505(2000)
\endreference

%%%\reference{cvdaa} A.~Coc \etal,
%%%\aj600,544(2004)
%%%\endreference

\reference{cyburt} R.H.~Cyburt,
\prD70,023505(2004)
\endreference

\reference{serpico} P.D.~Serpico \etal,
{JCAP}~{\bf 12}, 010 (2004) 
\endreference

\reference{boyd} R.N.~Boyd \etal,
\prD82,105005(2010)
\endreference

\reference{cd} R.H.~Cyburt and B.~Davids,
\prC78,012(2008)
\endreference

\reference{nbt} K.M.~Nollett \etal,
\ajl552,L1(2001)
\endreference

\reference{nh11} K.M.~Nollett and G.P.~Holder,
{\tt arXiv:1112.2683}\rm
\endreference

\reference{els} R.I.~Epstein \etal,
\nature263,198(1976)
\endreference

%\reference{schr} A.~Songaila \etal,
%\nature368,599(1994)
%\endreference

%\reference{*tfb} D.~Tytler, X.-M.~Fan, and  S.~Burles, 
%\nature381,207(1996)
%\endreference
%\reference{*bt} S.~Burles and D.~Tytler,
%\aj460,584(1996), \aj499,699(1998), \aj507,732(1998)
%\aj499,699(1998), \aj507,732(1998)
%\endreference
%\reference{*tyt} D.~Tytler \etal,
%Astron. J. {\bf 117}, 63 (1999)
%\endreference

%%%\reference{ome} J.M.~O'Meara \etal,
%%%\aj552,718(2001)
%%%\endreference

\reference{wood}
B.E. Wood \etal, \aj609,838(2004)
\endreference

\reference{dod} S.~D'Odorico \etal,
\aap368,L21(2001)
\endreference

\reference{rom2006} D.~Romano \etal,
\mnras369,295(2006)
\endreference

\reference{pb} M.~Pettini and D.~Bowen,
\aj560,41(2001) 
\endreference

%\reference{kirk} D.~Kirkman \etal,
%\ajs149,1(2003)
%\endreference

\reference{coo2013} R.~Cooke \etal,
{\tt arXiv:1308.3240}\rm
\endreference

%%\reference{ome06} J.M. O'Meara \etal,
%%\ajl649,L61(2006)
%%\endreference

%%\reference{pettini} M. Pettini \etal,
%%\mnras391,1499(2008)
%%\endreference

\reference{lev2002} S.A.~Levshakov \etal,
\aj565,696(2002)
\endreference

\reference{fum2011} M.~Fumagalli \etal,
\science334,1245(2011)
\endreference

\reference{sri2010} R.~Srianand \etal,
\mnras405,1888(2010) 
\endreference

\reference{not2012} P.~Noterdaeme \etal, 
\aap542,L33(2012)
\endreference

\reference{pet2012} M.~Pettini and R.~Cooke,
\mnras425,2477(2012) 
\endreference

%\reference{cwof} N.H.M. Crighton \etal,
% J.K. Webb, A. Ortiz-Gil \& A. Fernandez-Soto
%\mnras355,1042(2004)
%\endreference

%\reference{lin} J. Linsky, 
%Space Sci. Rev., {\bf 106}, 49 (2003)
%\endreference

%\reference{son} G. Sonneborn \etal, 
%\aj545,277(2000)
%\endreference

\reference{lin06} J.L. Linsky \etal,
\aj647,1106(2006)
\endreference

\reference{sav07} B.D. Savage \etal,
\aj659,1222(2007)
\endreference

%\reference{cla} D.D. Clayton,
%\aj290,428(1985)
%\endreference
%%\reference{fie} B.D. Fields, 
%%\aj456,678(1996)
%%\endreference

%%\reference{ktblo} D. Kirkman \etal,
%%\aj529,655(2000)
%%\endreference

%\reference{pste} B.E.J. Pagel \etal,
%\mnras255,325(1992)
%\endreference

\reference{izo} Y.I. Izotov \etal,
\aj527,757(1999)
\endreference

%\reference{fo98} B.D. Fields and K.A. Olive, 
%\aj506,177(1998)
%\endreference

%\reference{os} K.A. Olive \& E. Skillman,
%New Astron. {\bf 6}, 119 (2001)
%\endreference

\reference{os} K.A. Olive and E. Skillman,
\aj617,29(2004)
\endreference

%\reference{sj} D. Sauer & K. Jedamzik,
%astro-ph/0104392 %\aap?,?(2001) 
%\endreference

\reference{lppc} 
M. Peimbert \etal,
\aj667,636(2007)
%V. Luridiana \etal,
%\aj592,846(2003)
\endreference
%\reference{ppr} M. Peimbert \etal, %A. Peimbert \& M.T. Ruiz,
%\aj541,688(2000) 
%\endreference
%\reference{*ppl} A. Peimbert \etal, %M. Peimbert \& V. Luridiana,
%astro-ph/0107189 %\aj?,?(2001)
%\endreference

\reference{izo2} Y.I. Izotov \etal,
\aj662,15(2007)
\endreference

\reference{ave2012} E.~Aver \etal,
{JCAP}~{\bf 04}, 004 (2012)
\endreference

\reference{ave2013} E.~Aver \etal,
{\tt arXiv:1309.0047}\rm
\endreference

\reference{izo2013} Y.I.~Izotov \etal,
{\tt arXiv:1308.2100}\rm
\endreference

%\reference{izo2004} Y.I.~Izotov and T.X.~Thuan,
%\aj2004,602(2001)
%\endreference

%\reference{gus2011} N.G.~Guseva \etal,
%\aap529,149(2011)
%\endreference

\reference{trotta} R. Trotta and S.H. Hansen,
\prD69,023509(2004)
\endreference

\reference{PlanckCosmoParams} P.A.R.~Ade \etal\ (Planck Collaboration),
{\tt arXiv:1303.5076}\rm
\endreference

\reference{norbert} N. Christlieb \etal,
\nature419,904(2002)
\endreference

\reference{ss} M. Spite and F. Spite, 
\nature297,483(1982)
\endreference
%\reference{*tho} J.A. Thorburn,
%\aj412,318(1994)
%\endreference

%\reference{bm} P. Bonifacio \& P. Molaro, 
%\mnras285,847(1997)
%\endreference

%\reference{rnb} S.G. Ryan \etal, % J. Norris \& T. Beers,
%\aj523,654(1999)
%\endreference

%\reference{wssof} T.P. Walker \etal,
%\aj413,562(1993)
%\endreference

\reference{van} E. Vangioni-Flam \etal, 
New Astron. {\bf 4}, 245 (1999)
\endreference
%\reference{*fo4} B.D. Fields \& K.A. Olive, 
%New Astron. {\bf 4}, 255 (1999)
%\endreference

\reference{rbofn} S.G. Ryan \etal,
\ajl530,L57(2000)
\endreference

\reference{bon1997} P.~Bonifacio and P.~Molaro,
\mnras285,847(1997)
\endreference

\reference{boni}
P. Bonifacio \etal,
\aap390,91(2002)
\endreference

\reference{mel2010} J. Melendez \etal,
\aap515,L3(2010)
\endreference

\reference{boni07}
P. Bonifacio \etal,
\aap462,851(2007)
\endreference


%%\reference{mr}
%%J. Mel\'{e}ndez and I. Ramirez, 
%%\ajl615,33(2004)
%%\endreference

%\reference{vc} S. Vauclair \& C. Charbonnel,
%\aj502,372(1998)
%\endreference

\reference{umpli} W. Aoki,
\aj698,1803(2009)
\endreference
\reference{*hosford} A. Hosford \etal,
\aap493,601(2009)
\endreference

\reference{sbo} L. Sbordone \etal,
\aap522,A26(2010)
\endreference

\reference{caf2011} E.~Caffau \etal,
\nature477,67(2011)
\endreference

\reference{mol2012} P.~Molaro \etal,
{Memorie della Soc.~Astronomica Italiana Supp.} 22, 233 (2012)
\endreference

\reference{pswn} M.H. Pinsonneault \etal,
\aj574,389(2002)
\endreference

\reference{korn} A.J. Korn \etal,
\nature442,657(2006)
\endreference

\reference{asplund} M. Asplund \etal,
\aj644,229(2006)
\endreference

\reference{lin2013} K.~Lind \etal,
\aap554,96(2013)
\endreference

\reference{cayrel} R. Cayrel \etal,
\aap473,L37(2007)
\endreference

\reference{ste2012} M.~Steffen \etal,
{Memorie della Soc.~Astronomica Italiana Supp.} 22, 152 (2012)
\endreference

\reference{bbrw} T.M. Bania \etal,
\nature415,54(2002)
%D.S. Balser \etal,
%\aj510,759(1999)
\endreference

%\reference{gpsf} D. Galli \etal, 
%\ajl432,L101(1994)
%\endreference
\reference{osst} K.A. Olive \etal,
\aj479,752(1997)
\endreference

\reference{vofc} E. Vangioni-Flam \etal,
\aj585,611(2003)
\endreference

%\reference{tsof} E. Vangioni-Flam \etal,
%\aap360,15(2000)
%D. Thomas \etal,
%\aj406,569(1993)
%\endreference

\reference{rafs} H. Reeves \etal,
\aj179,909(1973)
\endreference

\reference{fhp} M. Fukugita and P.J.E. Peebles,
\aj616,643(2004)
%M. Fukugita \etal,
%\aj503,518(1998)
\endreference

%\reference{ho} D.J. Hegyi \& K.A. Olive,
%\aj303,56(1986) 
%\endreference
\reference{co} R. Cen and J.P. Ostriker,
\aj514,1(1999)
\endreference

\reference{jkks} G. Jungman \etal,
\prD54,1332(1996)
\endreference

%%\reference{tzh} M. Tegmark \etal,
%%\prD63,043007(2001)
%%\endreference

%\reference{kssw} J.P. Kneller \etal,
%\prD?,?(2001) 
%\endreference

%\reference{bgss} J. Barriga \etal,
%\mnras324,977(2001)
%\endreference

%\reference{wmap3} D.N. Spergel \etal,
%\ajs170,377(2007)
%\endreference
%\reference{*wmap1} D.N. Spergel \etal,
%\ajs148,175(2003)
%\endreference

%%\reference{wmap5} J. Dunkley \etal,
%%\ajs180,306(2009)
%%\endreference

\reference{coc2013} A.~Coc \etal,
{\tt arXiv:1307:6955}\rm(2013)
\endreference

\reference{cfo2} R.H. Cyburt \etal,
\plB567,227(2003)
\endreference

\reference{res} R.H.~Cyburt and M.~Pospelov, 
{Int.~J.~Mod.~Phys.~E}~{\bf 21}, 1250004 (2012) 
\endreference
\reference{*boy2010} R.N.~Boyd \etal,
\prD82,105005(2010)
\endreference
\reference{*cha2011} N. Chakraborty \etal,
\prD83,063006(2011)
\endreference
\reference{*bro2012} C. Broggini \etal,
{JCAP}~{\bf 06}, 030 (2012)
\endreference

\reference{oma2011} P.D.~O'Malley \etal,
\prC84,042801(2011)
\endreference

\reference{ric2005} O. Richard \etal,
\aj619,538(2005)
\endreference

\reference{gru2013} P.~Gruyters \etal,
{Astron.~Astrophys.}~{\bf 555}, 31 (2013)
\endreference

\reference{jr} K. Jedamzik and J.B. Rehm,
\prD64,023510(2001)  
\endreference

\reference{cobe} D.J. Fixsen \etal,
\aj473,576(1996)
\endreference

\reference{jed2004} K.~Jedamzik,
\prD70,063524(2004)
\endreference

\reference{kaw2005} M.~Kawasaki \etal,
\prD71,083502(2005)
\endreference

%\reference{varconst} J.P.~Uzan, 
%\rmp75,403(2003)
%\endreference
\reference{bar} J.D.~Barrow,
\prD35,1805(1987)
\endreference
\reference{*co95} B.A.~Campbell and K.A.~Olive,
\plB345,429(1995)
\endreference
\reference{*ber99} L.~Bergstr\"om,
\prD60,045005(1999)
\endreference
\reference{*fla} V.V.~Flambaum and E.V.~Shuryak,
\prd65,103503(2002)
\endreference
\reference{*coc2007} A.~Coc \etal,
\prD76,023511(2007)
\endreference
\reference{*ber2013} J.C.~Berengut \etal,
\prD87,085018(2013)
\endreference
%\reference{*coc12} A.~Coc \etal,
%\prD86,043529(2012)
%\endreference

%%\reference{hs} P. Hunt and S. Sarkar,
%%\prD76,123504(2007)
%%\endreference
%\reference{*bdrs} A. Blanchard \etal,
%\aap412,35(2003)
% astro-ph/0304237
%\endreference
%\reference{*bridle} S. Bridle \etal,
%\mnras342,L72(2003)
%\endreference

%\reference{hcw} G. Huey \etal,
%\prD69,103503(2005)
%\endreference

%\reference{zl} P.C. Stancil \etal,
%\aj580,29(2002)
%\endreference

\reference{ssg} G. Steigman \etal,
\plB66,202(1977)
\endreference

\reference{cfos} R.H. Cyburt \etal,
Astropart.~Phys.~{\bf 23}, 313 (2005)
\endreference

%\reference{ot} K.A. Olive \& D. Thomas,
%Astropart. Phys. {\bf 11}, 403 (1999)
%\endreference

\reference{lsv} E. Lisi \etal,
\prD59,123520(1999)
\endreference

%\reference{bnt} S. Burles \etal,
%\prl82,4176(1999);
%\prD63,063512(2001)
%\endreference

%\reference{magser} G. Mangano and P.D. Serpico,
%\plB701,296(2011)
%\endreference

\reference{hou2013} Z.~Hou \etal,
\prD87,083008(2013)
\endreference

\reference{spt} R. Keisler \etal,
\aj743,28(2011)
\endreference

\reference{darkrad} J.~Hamann \etal,
\prl105,181301(2010)
\endreference
%\reference{*arc2011} M.~Archidaicono \etal,
%\prD84,123008(2011) 
%\endreference
%\reference{*fis2011} W. Fishler and J. Meyers,
%\prD83,063520(2011)
%\endreference

%%\reference{barger} V. Barger \etal,
%%\plB566,8(2003)
%%\endreference

%\reference{barger2} V. Barger \etal,
%\plB569,123(2003)
%\endreference

\reference{kpw} E.W. Kolb \etal,
\prD33,869(1986)
\endreference
%\reference{*ds} V.V. Dixit \& M. Sher,
%\prD37,1097(1988)
%\endreference
\reference{*akr} F.S. Accetta \etal, 
\plB248,146(1990)
\endreference
%\reference{*ss} R.J. Scherrer \& D.N. Spergel,
%\prD47,4774(1993)
%\endreference
\reference{*co} B.A. Campbell and K.A. Olive,
\plB345,429(1995)
\endreference
%\reference{*bir} L. Bergstr\"om \etal,
%\prD60,045005(1999)
%\endreference
\reference{*nl} K.M. Nollett and R. Lopez,
\prD66,063507(2002)
\endreference
\reference{*bgv} C. Bambi \etal, % M. Giannotti \& F.L. Villante,
\prD71,123524(2005)
\endreference

\reference{couv} A. Coc \etal,
\prD73,083525(2006)
\endreference

\reference{oss81} K.A. Olive \etal, 
\npB180,497(1981)
\endreference

\reference{eens} J. Ellis \etal,
\plB167,457(1986)
\endreference

\reference{kta} L.M. Krauss \etal,
\prl71,823(1993) 
\endreference

\reference{mor} J.A. Morgan, 
\plB102,247(1981)
\endreference

\reference{ktw} E.W. Kolb \etal,
\prD34,2197(1986)
\endreference
\reference{*gm} J.A. Grifols and E. Mass\'o,
\mplA2, 205(1987)
\endreference
\reference{*bmr} K.S. Babu \etal,
\prl67,545(1991)
\endreference

\reference{dhs} A.D. Dolgov \etal,
\npB524,621(1998)
\endreference

\reference{ekt} K. Enqvist \etal,
\npB373,498(1992)
\endreference
\reference{*kc} A.D. Dolgov, 
\prept370,333(2002)
\endreference

\reference{gmr} J.A. Grifols \etal,
\plB400,124(1997)
\endreference

\reference{dhks} Dreiner \etal, 
\prD85,065027(2012)
\endreference

\reference{sk} K. Sato and M. Kobayashi,
\ptp58,1775(1977)
\endreference
\reference{*dktw} D.A. Dicus \etal,
\prD17,1529(1978)
\endreference 
\reference{*st98} R.J. Scherrer and M.S. Turner,
\aj331,19(1988)
\endreference

\reference{lin2} D. Lindley, 
\mnras188,15(1979);
\aj294,1(1985)
\endreference 

\reference{ens} J. Ellis \etal, % D.V. Nanopoulos \& S. Sarkar,
\npB259,175(1985)
\endreference
\reference{*eglns} J. Ellis \etal,
\npB373,399(1992)
\endreference
%\reference{*hkm} E. Holtmann, M. Kawasaki \& T. Moroi,
%\prD60,023506(1999) 
%\endreference
\reference{*cefo} R.H. Cyburt \etal,
\prD67,103521(2003)
\endreference

\reference{rs} M.H. Reno and D. Seckel,
\prD37,3441(1988)
\endreference
\reference{*dehs} S. Dimopoulos \etal,
%\aj330,545(1988),
\npB311,699(1989)
\endreference
%\reference{*koh} K. Kohri,
%\prD64,043515(2001)
\reference{*kkm} K. Kohri \etal,
\prD71,083502(2005)
\endreference

\reference{sc} S. Sarkar and A.M. Cooper,
\plB148,347(1984)
\endreference

%\reference{dgt} S. Dodelson \etal,
%\prD49,5068(1994)
%\endreference
%\reference{*kks} M. Kawasaki \etal,
%\plB430,132(1998)
%\endreference

\reference{pospelov} M. Pospelov \etal,
\prl98,231301(2007) 
\endreference
\reference{*kkm} M. Kawasaki \etal, 
\plB649,436(2007)
\endreference
\reference{*cefos} R.H. Cyburt \etal,
{JCAP}~{\bf 05}, 014 (2013) 
\endreference

\reference{jed} K. Jedamzik \etal,
{JCAP}~{\bf 07}, 007 (2006) 
\endreference

%\reference{eov} J. Ellis \etal,
%\plB619,30(2005)
%\endreference

\reference{davidson} S. Davidson \etal, 
\pr466,105(2008)
\endreference

\reference{wei2} S. Weinberg,
\prl48,1303(1979)
\endreference

\reference{bbb} M. Bolz \etal,
\npB606,518(2001)
\endreference

\reference{chrr} G. Coughlan \etal,
\plB131,59(1983)
\endreference

%\reference{bkn} T. Banks \etal,
%\prD49,779(1994)
%\endreference

\reference{ahdd} N. Arkani-Hamed \etal,
\prD59,086004(1999)
\endreference

\reference{rs2} L. Randall and R. Sundrum,
\prl83,3370(1999)
%\prl83,4690(1999)
\endreference

\reference{brane} J.M. Cline \etal,
\prl83,4245(1999)
\endreference
\reference{*bdel} P. Binetruy \etal,
\plB477,285(2000)
\endreference 

\endreferencelist


==> bigbangnuc-body.tex <==
\BleederPointer=7
\IndexEntry{bigbangnucpage}
%
\beginDBonly
\abovedisplayskip=\smallskipamount
        \belowdisplayskip=\smallskipamount
\endDBonly
%
\IndexEntry{bigbangnucpage}
%
\beginDBonly
\abovedisplayskip=\smallskipamount
%\belowdisplayskip=\smallskipamount
%\advance\baselineskip by -.6pt
\endDBonly
%
\ifnum\WhichSection=7
\magnification=\magstep1
\fi
%
\heading{BIG-BANG NUCLEOSYNTHESIS}
\runninghead{Big-Bang nucleosynthesis}
%
\beginRPPonly
\IndexEntry{bbnpage}
\overfullrule=5pt
%
% Redefine upper case greek letters so that particle names are slanted
% Make new definitions to correspond to old definitions
\mathchardef\OMEGA="700A
\mathchardef\Omega="700A
\WhoDidIt{Revised October 2013 by B.D.~Fields, (Univ.\ of Illinois) 
          P.~Molaro (Trieste Observatory) and S.~Sarkar (Univ.\ of Oxford 
          \& Niels Bohr Institute, Copenhagen).} % WhoDidIt

        Big-Bang nucleosynthesis (BBN) offers the deepest reliable
        probe of the early Universe, being based on well-understood
        Standard Model physics\cite{wfh}. Predictions of the
        abundances of the light elements, D, \he3, \he4, and \li7,
        synthesized at the end of the `first three minutes', are in
        good overall agreement with the primordial abundances inferred
        from observational data, thus validating the standard hot
        Big-Bang cosmology (see\refrange{st}{iocco} for reviews). This
        is particularly impressive given that these abundances span
        nine orders of magnitude -- from $\he4/\H \sim 0.08$ down to
        $\li7/\H \sim 10^{-10}$ (ratios by number). Thus BBN provides
        powerful constraints on possible deviations from the standard
        cosmology, and on new physics beyond the Standard
        Model\refrange{sar}{fie11}.

\section{Theory}

The synthesis of the light elements is sensitive to physical
conditions in the early radiation-dominated era at a temperature
$T \sim 1$~MeV, corresponding to an age $t \sim 1$~s. At higher
temperatures, weak interactions were in thermal equilibrium, thus
fixing the ratio of the neutron and proton number densities to be $n/p
= \rme^{-Q/T}$, where $Q = 1.293$~MeV is the neutron-proton mass
difference. As the temperature dropped, the neutron-proton
inter-conversion rate per nucleon, $\Gamma_{\np} \sim \,G_\F^2T^5$,
fell faster than the Hubble expansion rate,
$H \sim \sqrt{g_*G_\N} \;T^2$, where $g_*$ counts the number of
relativistic particle species determining the energy density in
radiation (see `Big Bang Cosmology' review). This resulted in
departure from chemical equilibrium (`freeze-out') at $T_\fr \sim
(g_*G_\N/G_{\rm F}^4)^{1/6} \simeq 1$~MeV. The neutron fraction at
this time, $n/p = \rme^{-Q/T_\fr} \simeq 1/6$, is thus sensitive to
every known physical interaction, since $Q$ is determined by both
strong and electromagnetic interactions while $T_\fr$ depends on the
weak as well as gravitational interactions. Moreover, the sensitivity
to the Hubble expansion rate affords a probe of, {\it e.g.,} the
number of relativistic neutrino species\cite{peeb}. After freeze-out,
the neutrons were free to $\beta$-decay, so the neutron fraction
dropped to $n/p \simeq 1/7$ by the time nuclear reactions began. A
simplified analytic model of freeze-out yields the $n/p$ ratio to an
accuracy of $\sim 1\%$\cite{bbf}\cite{m}.

The rates of these reactions depend on the density of baryons
(strictly speaking, nucleons), which is usually expressed normalized
to the relic blackbody photon density as $\eta \equiv
\,n_\b/n_\gamma$. As we shall see, all the light-element abundances
can be explained with $\eta_{10} \equiv \eta \times 10^{10}$ in the
range $5.7 \hbox{--} 6.7$ (95\%\ CL). With $n_\gamma$ fixed by the
present CMB temperature $2.7255 \,$K (see `Cosmic Microwave Background'
review), this can be stated as the allowed range for the baryon mass
density today, $\rho_\b = (3.9 \hbox{--} 4.6) \times
10^{-31}$~g\,cm$^{-3}$, or as the baryonic fraction of the critical
density, $\Omega_\b = \rho_\b/\rho_{\rm crit} \simeq \eta_{10}
h^{-2}/274 = (0.021 \hbox{--} 0.025) h^{-2}$, where $h \equiv
\,H_0/100 \ {\rm km \, s^{-1} \,Mpc^{-1}}$ is the
present Hubble parameter (see Cosmological Parameters review).

The nucleosynthesis chain begins with the formation of deuterium in
the process $p(n,\gamma)\D$. However, photo-dissociation by the high
number density of photons delays production of deuterium (and other
complex nuclei) until well after $T$ drops below the binding energy of
deuterium, $\Delta_\D = 2.23$~MeV. The quantity $\eta^{-1}
\rme^{-\Delta_\D/T}$, {\it i.e.,} the number of photons per baryon
above the deuterium photo-dissociation threshold, falls below unity at
$T\simeq 0.1$~MeV; nuclei can then begin to form without being
immediately photo-dissociated again. Only 2-body reactions, such as
$\D (p, \gamma) \he3$, $\he3 (\D, p) \he4$, are important because the
density by this time has become rather low -- comparable to that of
air!

Nearly all neutrons end up bound in the most stable light
element \he4. Heavier nuclei do not form in any significant quantity
both because of the absence of stable nuclei with mass number 5 or 8
(which impedes nucleosynthesis via $n \he4$, $p \he4$ or $\he4 \he4$
reactions), and the large Coulomb barriers for reactions such as $\he3
(\he4, \gamma) \li7$ and $\he3 (\he4, \gamma) \be7$. Hence the
primordial mass fraction of \he4, $Y_\p \equiv \rho(\he4)/\rho_{\rm
b}$, can be estimated by the simple counting argument
$$ 
%\RPPdisplaylines{
Y_\p = {2(n/p) \over 1+n/p} \simeq 0.25 \period \EQN {Yp}
%\cr} 
$$ 
There is little sensitivity here to the actual nuclear reaction rates,
which are, however, important in determining the other `left-over'
abundances: D and \he3 at the level of a few times $10^{-5}$ by number
relative to H, and \li7/H at the level of about $10^{-10}$ (when
$\eta_{10}$ is in the range $1 \hbox{--} 10$). These values can be
understood in terms of approximate analytic
arguments\cite{m}\cite{esd}.  The experimental parameter most
important in determining $Y_\p$ is the neutron lifetime, $\tau_n$,
which normalizes (the inverse of) $\Gamma_{\np}$.
% (This is not fully determined by $G_\F$ alone since neutrons and
% protons also have strong interactions, the effects of which cannot
% be calculated very precisely.)
Its value has recently been significantly revised downwards to $\tau_n
= 880.0
\pm 0.9$~s (see $N$ Baryons Listing).

The elemental abundances shown in \Fig{abundantlight} as a function of
$\eta_{10}$ were calculated\cite{cfo5} using an updated
version\cite{cfo} of the Wagoner code\cite{wfh}; other
versions\refrange{kaw}{alterBBN} are publicly available.
%\cite{sark}.
The \he4 curve includes small corrections due to radiative processes
at zero and finite temperatures\cite{emmp}, non-equilibrium neutrino
heating during $e^\pm$ annihilation\cite{dt}, and finite nucleon mass
effects\cite{seckel}; the range reflects primarily the 2$\sigma$
uncertainty in the neutron lifetime. The spread in the curves for
D, \he3, and \li7 corresponds to the 2$\sigma$ uncertainties in
nuclear cross sections, as estimated by Monte Carlo
methods [\use{Ref.cfo},\use{Ref.skm}--\use{Ref.coc}]. 
The input nuclear data have been carefully
reassessed [\use{Ref.cfo5},
\use{Ref.coc}--\use{Ref.boyd}], 
leading to improved precision in the
abundance predictions.  In particular, the uncertainty in \li7/H at
interesting values of $\eta$ has been reduced recently by a factor
$\sim 2$, a consequence of a similar reduction in the error budget
\cite{cd} for the dominant mass-7 production channel
$\he3(\he4,\gamma)\be7$. Polynomial fits to the predicted abundances
and the error correlation matrix have been
given\cite{flsv}\cite{nbt}. The boxes in \Fig{abundantlight} show the
observationally inferred primordial abundances with their associated
uncertainties, as discussed below.
%%\vskip -0.1in
\midfigure{abundantlight}
\RPPfigurescaled{bbnfig_13.eps}{center}{6.0in} {The abundances of
  \he4, D, \he3, and \li7 as predicted by the standard model of
  Big-Bang nucleosynthesis --- the bands show the 95\%\ CL
  range.  Boxes indicate the observed light element abundances.
  %%(smaller boxes: $\pm 2\sigma$ statistical errors; larger boxes:
  %%$\pm 2\sigma$ statistical {\it and} systematic errors).
  The narrow
  vertical band indicates the CMB measure of the cosmic baryon
  density, while the wider band indicates the BBN concordance range
  (both at $95\%$ CL). } %%%\twentyTenColorFig } 
\IndexEntry{bigbangnucOnePage}
\endfigure

The nuclear reaction cross sections important for BBN have all been
measured at the relevant energies. We will see, however, that recently
there have been substantial advances in the precision of light element
observations (e.g., D/H ) and in cosmological parameters (e.g., from
{\it Planck}).  This motivates corresponding improvement in BBN
precision and thus in the key reaction cross sections.  For example,
it has been suggested \cite{nh11} that $d(p,\gamma)\he3$
measurements may suffer from systematic errors and be inferior to {\it
ab initio} theory; if so, this could alter D/H abundances at a level
that is now significant.


\vfill\supereject
%% \sectionminspace=0.5in
\section{Light Element Abundances}
%% \sectionminspace=1in

BBN theory predicts the universal abundances of D, \he3, \he4, and
\li7, which are essentially fixed by $t\sim180$~s. Abundances
are, however, observed at much later epochs, after stellar
nucleosynthesis has commenced. This produces heavy elements such as C,
N, O, and Fe (`metals'), while the ejected remains of this stellar
processing alters the light element abundances from their primordial
values. Thus, one seeks astrophysical sites with low metal abundances,
in order to measure light element abundances that are closer to
primordial.  For all of the light elements, systematic errors are the
dominant limitation to the precision with which primordial abundances
can be inferred.

BBN is the only significant source of deuterium, which is entirely
destroyed when it is cycled into stars\cite{els}.  Thus, any detection
provides a lower limit to primordial D/H, and an upper limit on
$\eta_{10}$; for example, the local interstellar value of ${\rm D/H}
= (1.56 \pm 0.40) \times 10^{-5}$\cite{wood} requires $\eta_{10} \le
9$. The best proxy to the primordial value of D is its measure in
distant and chemically unprocessed matter where stellar processing
(astration) is minimal \cite{els}.  This has become possible with the
advent of large telescopes, but after two decades of observational
efforts we have only about a dozen determinations
\refrange{dod}{pet2012}.
High-resolution spectra reveal the presence of D in high-redshift,
low-metallicity quasar absorption systems via its isotope-shifted
Lyman-$\alpha$ absorption features; these are, unfortunately, usually
obscured by the Lyman-$\alpha$ forest.  The available D measurements
are performed in systems with metallicities from 0.1 to 0.001 Solar
where no significant astration is expected \cite{rom2006}. In the
best-measured systems, D/H shows no hint of correlation with
metallicity, redshift or the hydrogen column density $N({\rm H})$ (=
$\int_{\rm los} n_{\rm H} \ ds$) integrated over the line-of-sight
through the absorber. This is consistent with the measured D/H being
representative of the primordial value.
%An early claim of a trend with metallicity by [Kirkman et al 2003)]
%vanished with more measurements.  However, concern remains over
%systematic errors, the dispersion between the values being much
%larger than is expected from the individual measurement errors. Most
%of the problem arise in the determination of the hydrogen column in
%Lyman Limit systems due to the difficulty of dealing with
%photoionization.

The first measurements in `damped' Lyman-$\alpha$ systems (DLAs:
$N({\rm H}) > 10^{20} \ \rm cm^{-2}$) [\use{Ref.dod},\use{Ref.pb}]
showed that D/H can be measured in this class of absorbers where the
Lorentzian damping wings of Lyman-$\alpha$ and Lyman-$\beta$ (if
relatively uncontaminated by Lyman-$\alpha$ clouds) provide a precise
H column density.  Subsequently DLA systems have been found that also
show resolved higher members of the Lyman series. Systems with a
particularly simple kinematic structure are desirable to avoid
uncertainties with complex, only partially resolved components.
Recently a DLA showing 13 resolved D~{\eightrm I} absorption lines has
been analyzed together with 4 other suitable systems.
%using a new software tool to marginalize the fitting to the continuum
%and zero levels \cite{coo2013}.
This provides a strikingly improved precision over earlier work, with
a weighted mean of $\log({\rm D/H})=-4.597 \pm 0.006$, corresponding
to
$$
%\RPPdisplaylines{
{\rm D/H}|_{\rm p} = (2.53 \pm 0.04) \times 10^{-5} .\EQN{D}
%\cr}
$$

D/H values in the Galaxy show an unexpected scatter of a factor of
$\sim 2$ \cite{lin06}, with a bimodal distribution as well as an
anti-correlation with metal abundances. This suggests that
interstellar D not only suffers stellar astration but also partly
resides in dust particles that evade gas-phase observations. This is
supported by a measurement in the lower halo \cite{sav07}, which
indicates that the Galactic D abundance has decreased by a factor of
only $1.1 \pm 0.13$ since its formation. However in the DLA the dust
content is apparently quite small; this is implied by the abundances
of refractory elements such as Fe, Cr and Si, which are in nearly
Solar proportions.  Thus, the value derived in \Eq{D} appears safe
against D depletion into dust grains.

%[comment: the small amount of Li astration is a problem ... there is
%a tension between the Galactic high value of 23.1 +/- 2.4 ppm and the
%QSOs value of 25.3 +/- 0.004 since they coincide within the
%errors. 

The primordial \he4 abundance is best determined through recombination
emission lines of He and H in the most metal-poor extragalactic \hii\
(ionized) regions, {\it viz.} blue compact galaxies. There is now a
large body of data on \he4 and CNO in these galaxies, with over 1000
such systems in the Sloan Digital Sky Survey alone
[\use{Ref.izo},\use{Ref.izo2013}].  These data confirm that the small
stellar contribution to the helium abundance is positively correlated
with metal production, so extrapolation to zero metallicity gives the
primordial \he4 abundance $Y_\p$.  However, \hii\ regions are complex
systems and several physical parameters enter in the He/H
determination, notably the electron density and temperature, as well
as reddening. Thus systematic effects dominate the uncertainties in
the abundance determination [\use{Ref.izo},\use{Ref.os}].  In recent
work that has accounted for the underlying \he4\ stellar absorption,
and/or the newly derived values of the HeI-recombination and
H-excitation-collisional coefficients, the \he4 abundances have
significantly increased.  Some recent results are: $\Yp = 0.249 \pm
0.009$ \cite{os}; $\Yp = 0.248 \pm 0.003$ \cite{lppc}; $\Yp =
0.254 \pm 0.003$ or $0.252 \pm 0.001$ (depending on which set of He I
emissivities are used) \cite{izo2}; $\Yp = 0.2534 \pm
0.0083$ \cite{ave2012}; and $\Yp = 0.2465 \pm 0.0097$ \cite{ave2013}.
In the first and last two determinations the quoted error is a
conservative estimate of the systematic
uncertainties. Ref.~\cite{izo2013} used a subsample of 111 \hii\
regions drawn from a sample of 1610 objects,
%comprising the 3 most used samples, (the
%HeBCD \cite{izo2004} %%[Izotov Thuan 2004],
%VLT \cite{gus2011} %%[Guseva et al 2011] and SDSS R7)
as those providing $Y$ with an accuracy better than 3\%; the linear
regression in $Y-{\rm O/H}$ gives $\Yp = 0.254 \pm 0.0006\ ({\rm
stat}) \pm 0.003\ ({\rm syst})$.  
% Thus recent measurements are converging towards $\Yp =0.254$, but
% with estimates of the systematic error differing by a factor of 3.
% In Fig. 1.1 we show both estimates for the systematic error.
Our recommended \he4 abundance is 
$$ 
%\RPPdisplaylines{ 
Y_\p = 0.2465 \pm 0.0097 ,\EQN{Yp} 
%\cr}
$$
where we have adopted the result of the recent analysis
with the most detailed error budget \cite{ave2013}. 
Note that it does not
find a significant growth of $Y_\p$ with O/H.
%Averaging these values gives $Y_\p = 0.2535 \pm 0.0036$, in good
%agreement with the central value of \cite{izo2013}.

The CMB damping tail is sensitive to the primordial \he4 abundance,
and is independent from both BBN and local \he4 measurements.
\cite{trotta}.  Recent measurements yield 
$\Yp = 0.266 \pm 0.021$ (see Cosmic Microwave Background
review) \cite{PlanckCosmoParams}, {\it i.e.}, consistent with
the \hii\ region helium abundance determination.

As we will see in more detail below, the primordial abundance of
\li7 now plays a central role in BBN, and possibly points to new
physics. The systems best suited for Li observations are metal-poor
(Pop II) stars in the spheroid of the Galaxy, which have metallicities
going down to perhaps $10^{-5}$ of the solar value
\cite{norbert}. Observations have long shown 
\refrange{ss}{bon1997}  
that Li does not vary significantly in Pop II stars with metallicities
$\la 1/30$ of Solar --- the `Spite plateau' \cite{ss}. However there
are systematic uncertainties due to different techniques used to
determine the physical parameters ({\it e.g.}, the temperature) of the
stellar atmosphere in which the Li absorption line is
formed. Different analyses and in some cases different stars and
stellar systems (globular clusters), yield ${\rm Li/H}|_{\rm p} =
(1.7 \pm 0.3) \times 10^{-10}$
\cite{bon1997}, 
${\rm Li/H}|_{\rm p} = (2.19 \pm 0.28) \times 10^{-10}$
\cite{boni}, and
${\rm Li/H}|_{\rm p} = (1.86 \pm 0.23) \times 10^{-10}$
\cite{mel2010}.

Recent observations find a puzzling drop in Li/H in metal-poor stars
with $[{\rm Fe/H}] \equiv \log_{10}[({\rm Fe/H})/({\rm Fe/H})_\odot] <
-3.0$ [\use{Ref.boni07},\use{Ref.umpli},\use{Ref.sbo}].  In particular
Li is not detected in the two metal poor dwarfs with metallicities of
$[{\rm Fe/H}] \la -5$ (HE 1327$-$2326 and SDSS J102915+172927 where
${\rm Li/H} < 10^{-11}$) suggesting that something is depleting Li at
very low metallicity \cite{caf2011}. Since these stars have small
masses and are almost fully convective during pre-main sequence
evolution, they could have burned some Li \cite{mol2012}. The same
effect may produce the melting of the Li plateau at low metallicities
[\use{Ref.umpli},\use{Ref.sbo}] thus making quite uncertain any
primordial Li value obtained by extrapolating to zero
metallicity. Hence to estimate ${\rm Li/H}|_{\rm p}$ it is safer to
consider stars with $-2.8 <[{\rm Fe/H}]<-1.5$ \cite{sbo} which
provides
$$ 
%\RPPdisplaylines{ 
{\rm Li/H}|_\p = (1.6\pm 0.3) \times 10^{-10} .\EQN{Li}
%\cr}
$$
Moreover, the Li in Pop II stars may have been partially destroyed due
to mixing of the outer layers with the hotter
interior \cite{pswn}. Such processes can be constrained by 
observations of the fragile isotope \li6 \cite{van}, and by the
absence of significant scatter in Li versus Fe \cite{rbofn}.  Li
depletion by a factor as large as $\sim 1.8$ has been
suggested \cite{korn}.

Stellar determination of Li abundances typically sum over both stable
isotopes \li6 and \li7. Recent high-precision measurements are
sensitive to the tiny isotopic shift in Li absorption (which manifests
itself in the shape of the blended, thermally broadened line) and
indicate $\li6/\li7 \le 0.05$ [\use{Ref.asplund},\use{Ref.lin2013}],
thus confirming that \li7 is dominant. A claim of a \li6 plateau
(analogous to the \li7 plateau) has been made \cite{asplund},
suggesting a significant primordial \li6 abundance. This has, however,
been challenged by new observations and analyses
[\use{Ref.cayrel},\use{Ref.ste2012},\use{Ref.lin2013}], which show
that stellar convective motions can generate asymmetries in the line
shape that mimic the presence of \li6. Hence the deduced abundance
ratio $\li6/\li7 < 0.05$ in the best studied stars presently provides
a robust upper limit on the \li6 abundance \cite{lin2013}.

Turning to \he3, the only data available are from the Solar system and
(high-metallicity) \hii\ regions in our Galaxy\cite{bbrw}.  This makes
inferring the primordial abundance difficult, a problem compounded by
the fact that stellar nucleosynthesis models for \he3 are in conflict
with observations\cite{osst}.  Consequently, it is no longer
appropriate to use \he3 as a cosmological probe; instead, one might
hope to turn the problem around and constrain stellar astrophysics
using the predicted primordial \he3 abundance\cite{vofc}.


\section{Concordance, Dark Matter, and the CMB} 

We now use the observed light element abundances to test the theory.
We first consider standard BBN, which is based on Standard Model
physics alone, so $\nnu = 3$ and the only free parameter is the
baryon-to-photon ratio $\eta$. (The implications of BBN for physics
beyond the Standard Model will be considered below, \Section{sect:bbnbsm}). Thus,
any abundance measurement determines $\eta$, and additional
measurements overconstrain the theory and thereby provide a
consistency check.

% First we note that the overlap in the $\eta$ ranges spanned by the
% larger boxes in \Fig{abundantlight} indicates overall
% concordance. More quantitatively, when we account for theoretical
% uncertainties, as well as the statistical and systematic errors in
% observations, there is acceptable agreement among the abundances
% when $$ %\RPPdisplaylines{ 5.7 \le \eta_{10} \le 6.7 \ (95\%\ {\rm
% CL}), \EQN{etarange} %\cr} $$ a narrow range, due entirely to the
% very tight D/H precision.  However, the agreement is much less
% satisfactory if we use only the quoted statistical errors in the
% observations. In particular, as seen in \Fig{abundantlight}, D
% and \he4 are consistent with each other, but favor a value of $\eta$
% which is higher by a factor of at least 2.4, and by at least
% $\sim4.2\sigma$ from that indicated by the \li7 abundance determined
% in stars. Additional studies are required to %clarify if this
% discrepancy is real. Furthermore, if the \li6 plateau\cite{asplund}
% reflects a primordial component, it is $\sim1000$ times that
% expected in standard BBN; both these ``lithium problems'' may
% indicate new physics (see below).

While the $\eta$ ranges spanned by the boxes in \Fig{abundantlight} do
not all overlap, they are all within a factor $\sim 2$ of each
other. In particular, the lithium abundance corresponds to $\eta$
values that are inconsistent with that of the (now very precise) D/H
abundance as well as the less-constraining \he4 abundance. This
discrepancy marks the ``lithium problem''. The problem could simply
reflect difficulty in determining the primordial lithium abundance; or
could hint at a more fundamental omission in the theory.  The
possibility that lithium reveals new physics is addressed in detail in
the next section.  If however we exclude the lithium constraint
because its inferred abundance may suffer from systematic
uncertainties, then D/H and \he4 are in agreement.  The concordant
$\eta$ range is essentially that implied by D/H, namely
$$ 
%\RPPdisplaylines{
5.7 \le \eta_{10} \le 6.7 \ (95\%\ {\rm CL}). \EQN{etarange}
%\cr} 
$$ 
Despite the lithium problem, the overall concordance remains
remarkable: using only well-established microphysics we can
extrapolate back to $t \sim 1$~s to predict light element abundances
spanning 9 orders of magnitude, in approximate agreement with
observation.  This is a major success for the standard cosmology, and
inspires confidence in extrapolation back to still earlier times.

This concordance provides a measure of the baryon content: 
$$
%\RPPdisplaylines{
0.021 \le \Omega_\b h^2 \le 0.025 \ (95\%\ {\rm CL}) , \EQN{OmegaB}
%\cr} 
$$ 
a result that plays a key role in our understanding of the matter
budget of the Universe. First we note that $\Omega_\b \ll 1$, {\it
i.e.}, baryons cannot close the Universe\cite{rafs}. Furthermore, the
cosmic density of (optically) luminous matter is $\Omega_\l
\simeq 0.0024 h^{-1}$\cite{fhp}, so that $\Omega_\b \gg \Omega_\l$: 
most baryons are optically dark, probably in the form of a
diffuse intergalactic medium\cite{co}. Finally,
given that $\Omega_\m \sim 0.3$ (see Dark Matter and
Cosmological Parameters reviews), we infer that most matter in the
Universe is not only dark, but also takes some non-baryonic (more
precisely, non-nucleonic) form.

The BBN prediction for the cosmic baryon density can be tested through
precision observations of CMB temperature fluctuations (see Cosmic
Microwave Background review). One can determine $\eta$ from the
amplitudes of the acoustic peaks in the CMB angular power
spectrum\cite{jkks}, making it possible to compare two measures of
$\eta$ using very different physics, at two widely separated
epochs. In the standard cosmology, there is no change in $\eta$
between BBN and CMB decoupling, thus, a comparison of $\eta_\BBN$ and
$\eta_\CMB$ is a key test. Agreement would endorse the standard
picture,
% , and would open the way to sharper understanding of particle
% physics and astrophysics.
while disagreement could point to new physics during/between the BBN
and CMB epochs.

% The release of the WMAP results was a landmark event in this test of
% BBN. As with other cosmological parameter determinations from CMB
% data, the derived $\eta_\CMB$ depends on the adopted
% priors\cite{tzh}, in particular the form assumed for the power
% spectrum of primordial density fluctuations. If this is taken to be
% a scale-free power-law, the five-year WMAP data imply %
% $\Omega_{\B}h^2 = 0.0219 \pm 0.0007$ or $\eta_{10} = 5.98 \pm
% 0.25$, % while allowing for a ``running'' spectral index changes the
% value to $\Omega_{\b}h^2 = 0.02273 \pm 0.00062$ or $\eta_{10} =
% 6.23 \pm 0.17$\cite{wmap5} as shown in \Fig{abundantlight}. Other
% assumptions for the shape of the power spectrum can lead to baryon
% densities as low as $\Omega_\b h^2 = 0.0175 \pm
% 0.0007$\cite{hs}. Thus, outstanding uncertainties regarding priors
% are a source of systematic error which presently exceeds the
% statistical error in the prediction for $\eta$.

The analysis described in the Cosmic Microwave Background review,
based on recent {\it Planck} data, yields $\Omega_{\b}h^2 =
0.02207 \pm 0.00027$ or $\eta_{10} = 6.047 \pm
0.074$ \cite{PlanckCosmoParams}. As shown in
\Fig{abundantlight}, this CMB estimate of the baryon density (narrow
vertical band) is remarkably consistent with the BBN range quoted
in \Eq{OmegaB} and thus in very good agreement with the value inferred
from recent high-redshift D/H measurements\cite{coo2013} and \he4
determinations; together these observations span diverse environments
from redshifts $z= 1000$ to the present \cite{coc2013}.

%%%Bearing in mind the importance of priors, 
The precision determinations of the baryon density using the CMB
motivates the use of this value as an input to BBN
calculations. Within the context of the Standard Model, BBN then
becomes a zero-parameter theory, and the light element abundances are
completely determined to within the uncertainties in $\eta_\CMB$ and
the BBN theoretical errors. Comparison with the observed abundances
then can be used to test the astrophysics of post-BBN light element
evolution\cite{cfo2}.  Alternatively, one can consider possible
physics beyond the Standard Model ({\it e.g.}, which might change the
expansion rate during BBN) and then use all of the abundances to test
such models; this is discussed in \Section{sect:bbnbsm}.

\section{The Lithium Problem}

As \Fig{abundantlight} shows, stellar Li/H measurements are
inconsistent with the CMB (and D/H), given the error budgets we have
quoted.  Recent updates in nuclear cross sections and stellar
abundance systematics {\it increase} the discrepancy to over
$5\sigma$, depending on the stellar abundance analysis
adopted \cite{cfo5}.

The question then becomes pressing as to whether this mismatch comes
from systematic errors in the observed abundances, and/or
uncertainties in stellar astrophysics or nuclear inputs, or whether
there might be new physics at work\cite{fie11}. Nuclear inputs (cross
sections) for BBN reactions are constrained by extensive laboratory
measurements; to increase \be7 destruction requires enhancement of
otherwise subdominant processes that can be attained by missed
resonances in a few reactions such as $\be7(d,p)2\alpha$ if the
compound nuclear state properties are particularly
favorable \cite{res}.  However, experimental searches have now closed
off the most promising of these cases \cite{oma2011}, making a
``nuclear fix'' increasingly unlikely.

Another conventional means to solve the lithium problem is by {\it in
situ} destruction over the long lifetimes of the host halo stars.
Stellar depletion mechanisms include diffusion, rotationally induced
mixing, or pre-main-sequence depletion. These effects certainly occur,
but to reduce lithium to the required levels generally requires some
{\it ad hoc} mechanism and fine tuning of the initial stellar
parameters [\use{Ref.mol2012},\use{Ref.ric2005}].
%%%[Richard, Michaud, & Richer (2005) ApJ 619, 538,; Ref 71].  
A putative signature of diffusion has been reported for the globular
clusters NGC 6397 and NGC 6752, where the `turnoff' stars exhibit
slightly lower (by $\sim 0.1$ dex) abundances of Fe~{\eightrm II},
Ti~{\eightrm II}, Sc~{\eightrm II}, Ca~{\eightrm I} and Mg~{\eightrm
I}, than in more evolved stars
%%%Refs.~[67 and Gruyters et al 2013 A&A 555, A31) 
[\use{Ref.korn},\use{Ref.gru2013}].  General features of diffusive
models are a dispersion in the Li abundances and a pronounced downturn
in the Li abundances at the hot end of the Li plateau. Some extra
turbulence needs to be invoked to limit diffusion in the hotter stars
and to restore uniform Li abundance along the Spite
plateau \cite{ric2005}. In the framework of these models (and also
assuming identical initial stellar rotation) depletion by at most a
factor $\sim 1.8$ is conceivable [\use{Ref.korn},\use{Ref.gru2013}].

As nuclear and astrophysical solutions to the lithium problem become
increasingly constrained (even if difficult to rule out definitively),
the possibility of new physics arises.  Nucleosynthesis models in
which the baryon-to-photon ratio is inhomogeneous can alter abundances
for a given $\eta_\BBN$, but will overproduce \li7\cite{jr}.  Entropy
generation by some non-standard process could have decreased $\eta$
between the BBN era and CMB decoupling, however the lack of spectral
distortions in the CMB rules out any significant energy injection upto
a redshift $z \sim 10^7$\cite{cobe}.  The most intriguing resolution
of the lithium problem thus involves new physics during
BBN \refrange{jedpos}{fie11}.

We summarize the general features of such solutions here, and later
consider examples in the context of specific particle physics models.
Many proposed solutions introduce perturbations to light-element
formation during BBN; while all element abundances may suffer
perturbations, the interplay of \li7 and D is often the most important
{\it i.e.} observations of D often provide the strongest constraints
on the allowed perturbations to \li7.  In this connection it is
important to note that the new, very precise determination of ${\rm
D/H}$ \cite{coo2013} will significantly constrain the ability of such
models to ameliorate or solve the lithium problem.

A well studied class of models invokes the injection of suprathermal
hadronic or electromagnetic particles due to decays of dark matter
particles.  The effects are complex and depend on the nature of the
decaying particles and their branchings and spectra. However, the
models that most successfully solve the lithium problem generally
feature non-thermal nucleons, which dissociate all light elements.
Dissociation of even a small fraction of \he4 introduces a large
abundance of free neutrons, which quickly thermalize.  The thermal
neutrons drive the $\be7(n,p)\li7$ conversion of \be7.  The
resulting \li7 has a lower Coulomb barrier relative to
\be7 and is readily destroyed via $\li7(p,\alpha)\he4$
[\use{Ref.jed2004},\use{Ref.kaw2005}].  
But \he4 dissociation also produces D directly and via nonthermal
neutron $n(p,\gamma)d$ reactions; this introduces a tension between
Li/H reduction and D/H enhancement.

Another important class of models retains the standard cosmic particle
content, but changes their interactions via time variations in the
fundamental constants \cite{bar}. Here too, the details are
model-dependent, but scenarios that solve or alleviate the lithium
problem often feature perturbations to the deuteron binding energy. A
weaker D binding leads to the D bottleneck being overcome later, so
that element formation commences at a lower temperature and lower
density. This leads in turn to slower nuclear rates that freeze out
earlier. The net result is a {\it higher} final D/H, due to less
efficient processing into \he4, but also {\it lower} Li, due to
suppressed production via $\he3(\alpha,\gamma)\be7$.

The lithium problem remains an unresolved issue in BBN. Nevertheless,
the remarkable concordance between the CMB and the D (as well as \he4)
abundance, remains a non-trivial success, and provides constraints on
the early Universe and particle physics.


\section{Beyond the Standard Model}
\labelsection{sect:bbnbsm}


Given the simple physics underlying BBN, it is remarkable that it
still provides the most effective test for the cosmological viability
of ideas concerning physics beyond the Standard Model. Although
baryogenesis and inflation must have occurred at higher temperatures
in the early Universe, we do not as yet have `standard models' for
these, so BBN still marks the boundary between the established and the
speculative in Big Bang cosmology. It might appear possible to push
the boundary back to the quark-hadron transition at $T \sim
\Lambda_{\rm QCD}$, or electroweak symmetry breaking at $T \sim
1/\sqrt{G_\F}$; however, so far no observable relics of these epochs
have been identified, either theoretically or observationally. Thus,
although the Standard Model provides a precise description of physics
up to the Fermi scale, cosmology cannot be traced in detail before the
BBN era.

Limits on new physics come mainly from
the observational bounds on the \he4 abundance. This is proportional
to the $n/p$ ratio when the weak-interaction rate
falls behind the Hubble expansion rate at $T_\fr \sim 1$~MeV. The
presence of additional neutrino flavors (or of any other relativistic
species) at this time increases $g_*$, hence the expansion rate,
leading to a larger value of $T_\fr$, $n/p$, and therefore
$Y_\p$\cite{peeb}\cite{ssg}.  In the Standard Model at $T=1$~MeV, $g_* = 5.5 +
{7\over4}N_\nu$, where $N_\nu$ is the {\it effective} number of (nearly)
massless neutrino flavors (see Big Bang Cosmology review). The helium
curves in \Fig{abundantlight} were computed taking $N_\nu = 3$; small
corrections for non-equilibrium neutrino heating\cite{dt} are included
in the thermal evolution and lead to an effective $N_\nu = 3.04$
compared to assuming instantaneous neutrino freezeout (see Big
Bang Cosmology review).  The computed \he4 abundance scales as
$\Delta\,Y_\p \simeq 0.013 \Delta\nnu$\cite{bbf}. Clearly the central
value for $N_\nu$ from BBN will depend on $\eta$, which is
independently determined (with weaker sensitivity to $\nnu$) by the
adopted D or \li7 abundance. For example, if the best value for the
observed primordial \he4 abundance is 0.249, then, for $\eta_{10} \sim
6$, the central value for $N_\nu$ is very close to 3. 
%This limit depends sensitively on the adopted light element abundances, particularly $Y_\p$.  
A maximum likelihood analysis on $\eta$ and
$N_\nu$ based on the above \he4 and D abundances finds the
(correlated) 95\% CL ranges to be $4.9 < \eta_{10} < 7.1$ and $1.8 <
\nnu < 4.5$\cite{cfos}.  
% On the other hand, using the `low' \he4 and \li7 gives\cite{ot}
% $\eta_{10} \le 4.3$, and $1.4 \le \nnu \le 4.9$.
Identical results are obtained using a simpler method to extract such bounds based on $\chi^2$
statistics, given a set of input abundances \cite{lsv}.
% Tighter bounds are obtained if less conservative assumptions are
% made concerning primordial abundances, e.g. adopting the D
% abundance \cite{ome} fixes $\eta_{10} = 5.6 \pm 0.6$
% ($\Omega_{\B}h^2 = 0.02 \pm 0.002$) at 95\% CL.  , and requires
% $\nnu < 3.2$\cite{bnt} even if the `high' \he4 abundance\cite{izo}
% is used.

The CMB power spectrum in the damping tail is independently
sensitive to $\nnu$ ({\it e.g.} \cite{hou2013}). The CMB value
$\nnu^{\rm CMB}$ probes the cosmic radiation content at (re)combination,
so a discrepancy would imply new physics or astrophysics. Indeed, observations by the South
Pole Telescope implied $\nnu^{\rm CMB} = 3.85 \pm 0.62$\cite{spt},
prompting discussion of ``dark radiation'' such as sterile
neutrinos \cite{darkrad}. However, recent {\it Planck} results give
$\nnu^{\rm CMB} = 3.36^{+0.34}_{-0.32}$ with a precision now apparently better
than BBN, which is quite consistent with the Standard Model
[\use{Ref.PlanckCosmoParams}]. If we {\it assume} that $\eta$ did not change between BBN and (re)combination, the constraint can be improved by including the recent D/H measurements, which yields $\nnu = 3.28 \pm 0.28$ \cite{coo2013}.

Just as one can use the measured helium abundance to place limits on
$g_*$\cite{ssg}, any changes in the strong, weak, electromagnetic, or
gravitational coupling constants, arising \eg, from the dynamics of
new dimensions, can be similarly constrained\cite{kpw}, as can be any
speed-up of the expansion rate in, {\it e.g.}, scalar-tensor theories
of gravity\cite{couv}.

The limits on $N_\nu$ can be translated into limits on other types of
particles or particle masses that would affect the expansion rate of
the Universe during nucleosynthesis. For example, consider `sterile'
neutrinos with only right-handed interactions of strength $G_\R <
G_\F$. Such particles would decouple at higher temperature than
(left-handed) neutrinos, so their number density ($\propto \;T^3$)
relative to neutrinos would be reduced by any subsequent entropy
release, {\it e.g.}, due to annihilations of massive particles that
become non-relativistic between the two decoupling temperatures. Thus
(relativistic) particles with less than full strength weak
interactions contribute less to the energy density than particles that
remain in equilibrium up to the time of nucleosynthesis\cite{oss81}.
If we impose $\nnu < 4$ as an illustrative constraint, then the three
right-handed neutrinos must have a temperature
$3(T_{\nu_\R}/T_{\nu_\L})^4 < 1$. Since the temperature of the
decoupled $\nu_\R$ is determined by entropy conservation (see Big Bang
Cosmology review), $T_{\nu_\R}/T_{\nu_\L} =
[(43/4)/g_*(T_\d)]^{1/3}<0.76$, where $T_\d$ is the decoupling
temperature of the $\nu_\R$. This requires $g_*(T_\d) > 24$, so
decoupling must have occurred at $T_\d > 140$~MeV. The decoupling
temperature is related to $G_\R$ through $(G_\R/G_\F)^2 \sim
(T_\d/3\,{\rm MeV})^{-3}$, where 3~MeV is the decoupling temperature
for $\nu_\L$s. This yields a limit $G_\R \ltsim 10^{-2}G_\F$. The
above argument sets lower limits on the masses of new $Z'$ gauge
bosons to which right-handed neutrinos would be coupled in models of
superstrings\cite{eens}, or extended technicolor\cite{kta}. Similarly
a Dirac magnetic moment for neutrinos, which would allow the
right-handed states to be produced through scattering and thus
increase $g_*$, can be significantly constrained\cite{mor}, as can any
new interactions for neutrinos that have a similar effect\cite{ktw}.
Right-handed states can be populated directly by helicity-flip
scattering if the neutrino mass is large enough, and this property has
been used to infer a bound of $m_{\nu_\tau} \ltsim 1$~MeV taking $\nnu
< 4$\cite{dhs}. If there is mixing between active and sterile
neutrinos then the effect on BBN is more complicated\cite{ekt}.

BBN limits on the cosmic expansion rate constrain supersymmetric
scenarios in which the neutralino or gravitino are very light, so that they contribute
to $g_*$ \cite{gmr}. A gravitino in the mass range $\sim10^{-4} - 10$ eV will affect the expansion rate of the Universe similarly to a light neutralino (which is however now probably ruled out by collider data, especially the decays of the Higgs-like boson). The net contribution to $\nnu$ then ranges between 0.74 and 1.69, depending on the gravitino and slepton masses \cite{dhks}.

The limit on the expansion rate during BBN can also be translated into
bounds on the mass/lifetime of non-relativistic particles that decay
during BBN. This results in an even faster speed-up rate, and
typically also changes the entropy\cite{sk}. If the decays include
Standard Model particles, the resulting
electromagnetic\refrange{lin2}{ens} and/or hadronic\cite{rs} cascades
can strongly perturb the light elements, which leads to even stronger
constraints.  Such arguments had been applied to rule out an MeV mass
for $\nu_\tau$, which decays during nucleosynthesis\cite{sc}.
% ; even if the decay products are non-interacting particles (and
% lighter neutrinos), interesting bounds can be derived from
% considering their effects on BBN\cite{dgt}.

Decaying-particle arguments have proved very effective in probing
supersymmetry.  Light-element abundances generally are complementary
to accelerator data in constraining SUSY parameter space, with BBN
reaching to values kinematically inaccessible to the LHC.  Much recent
interest has focused on the case in which the next-to-lightest
supersymmetric particle is metastable and decays during or after BBN.
The constraints on unstable particles discussed above imply stringent
bounds on the allowed abundance of such particles\cite{rs}; if the
metastable particle is charged ({\it e.g.}, the stau), then it is
possible for it to form atom-like electromagnetic bound states with
nuclei, and the resulting impact on light elements can be quite
complex\cite{pospelov}.  Moreover, SUSY decays can destroy \li7 and/or
produce \li6, leading to a possible supersymmetric solution to the
lithium problems noted above\cite{jed} (see\cite{jedpos} for a
review).

These arguments impose powerful constraints on supersymmetric
inflationary cosmology\refrange{ens}{rs}, particularly thermal
leptogenesis\cite{davidson}.  These can be evaded only if the
gravitino is massive enough to decay before BBN, {\it i.e.}, $m_{3/2}
\gtsim 50$~TeV \cite{wei2} (which would be unnatural), or if it is in
fact the lightest supersymmetric particle and thus
stable\cite{ens}\cite{bbb}. Similar constraints apply to moduli --
very weakly coupled fields in string theory that obtain an
electroweak-scale mass from supersymmetry breaking\cite{chrr}.

Finally, we mention that BBN places powerful constraints on the
possibility that there are new large dimensions in nature, perhaps
enabling the scale of quantum gravity to be as low as the electroweak
scale\cite{ahdd}. Thus, Standard Model fields may be localized on a
`brane,' while gravity alone propagates in the `bulk.'  It has been
further noted that the new dimensions may be non-compact, even
infinite\cite{rs2}, and the cosmology of such models has attracted
considerable attention. The expansion rate in the early Universe can
be significantly modified, so BBN is able to set interesting
constraints on such possibilities\cite{brane}.
%
\smallskip
\noindent{\bf References:}
\smallskip
\parindent=20pt
\ListReferences
\endRPPonly
\vfill\eject
%
%
%\beginDBonly
%\smallskip
%\refline\parindent=20pt
%\endDBonly 
%


==> bigbangnuc-def.tex <==
%auto-ignore
%DEFINITIONS FOR BIG BANG NUCL

%\def\la{    \mathrel{\rlap{\raise 0.511ex
%        \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}
%\def\ga{    \mathrel{\rlap{\raise 0.511ex
%        \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}
\def\rme{{\rm e}}

\def\H{{\rm H}}
\def\D{{\rm D}}
\def\T{{\rm T}}
\def\Yp{Y_{\rm p}}
\def\be#1{\hbox{$^{#1}$Be}}
\def\he#1{\hbox{$^{#1}$He}}
\def\li#1{\hbox{$^{#1}$Li}}
\def\b1#1{\hbox{${}^{1#1}$B}}

\def\b{{\rm b}}
\def\BBN{{\rm BBN}}
\def\CMB{{\rm CMB}}
\def\d{{\rm d}}
\def\F{{\rm F}}
\def\fr{{\rm fr}}
\def\hii{H~{\eightrm II}}
\def\L{{\rm L}}
\def\l{{\rm lum}}
\def\m{{\rm m}}
\def\msol{\hbox{$M_{\odot}$}}
\def\N{{\rm N}}
\def\nnu{N_\nu}
\def\np{{n\!\leftrightarrow\!p}}
\def\p{{\rm p}}
\def\popii{Pop~{\eightrm II}}
\def\R{{\rm R}}
\def\stat{{\rm stat}}
\def\syst{{\rm syst}}
\def\yp{\hbox{$Y_{\rm p}$}}

\def\la{    \mathrel{\rlap{\raise 0.511ex
        \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

